Collaborative Coded Caching for Partially Connected Networks

Coded caching leverages the differences in user cache memories to achieve gains that scale with the total cache size, alleviating network congestion due to high-quality content requests. Additionally, distributing transmitters over a wide area can mitigate the adverse effects of path loss. In this work, we consider a partially connected network where the channel between distributed transmitters (helpers) and users is modeled as a distributed multiple-input-multiple-output (MIMO) Gaussian broadcast channel. We propose a novel delivery scheme consisting of two phases: partitioning and transmission. In the partitioning phase, users with identical cache profiles are partitioned into the minimum number of sets, such that users within each set can successfully decode their desired message from a joint transmission enabled by MIMO precoding. To optimally partition the users, we employ the branch and bound method. In the transmission phase, each partition is treated as a single entity, and codewords are multicast to partitions with distinct cache profiles. The proposed delivery scheme is applicable to any partially connected network, and while the partitioning is optimal, the overall delivery scheme, including transmission, is heuristic. Interestingly, simulation results show that its performance closely approximates that of the fully connected optimal solution.

==> conclusion.tex <==
%\textcolor{blue}{Look at 'Transmission'. Other than a simple summary of what we did, we should mention the non-optimality of our results and say we are improving the transmission in the future. Maybe for an optimal scheme, one should consider partitioning and transmission together, similar to Parinello cyclically permuting the partitions and then serving the partitions corresponding to users with different caches together. (But the extension from Parinello is not trivial because partitions are not uniform.)} % and we can not divide subfiles into smaller subfiles scaled with number of antennas since the users are not uniform, i.e., we have to serve some users more since they can be served in more partitions which implies we have to divide the requested file of that user into more subfiles which we can not do directly because we don't know which files users request. One has to check if dividing the files uniformly or nonuniformly into smaller subfiles depending on the number of antennas works or not.)}






%\textcolor{green}{References: Meixia Tao, Naderializadeh (probably also Avestimehr they have a paper about partially connected networks,}
